Section on Prospects for Dark Matter Detection of the White Paper on the Status and Future of Ground-Based TeV Gamma-Ray Astronomy

This is a report on the findings of the dark matter science working group for the white paper on the status and future of TeV gamma-ray astronomy. The white paper was commissioned by the American Physical Society, and the full white paper can be found on astro-ph (arXiv:0810.0444). This detailed section discusses the prospects for dark matter detection with future gamma-ray experiments, and the complementarity of gamma-ray measurements with other indirect, direct or accelerator-based searches. We conclude that any comprehensive search for dark matter should include gamma-ray observations, both to identify the dark matter particle (through the charac- teristics of the gamma-ray spectrum) and to measure the distribution of dark matter in galactic halos.

==> 8-references.tex <==
\begin{thebibliography}{10}
\setlength{\itemsep}{-0.0em}
\setlength{\parsep}{4pt}
\setlength{\baselineskip}{13pt}

\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}

% BEGIN REFS SNR

\bibitem{hillas05} Hillas, A.M., J.\ Phys.\ G: Nucl.\ Part.\ Phys. {\bf 31}, R95. (2005)

\bibitem{Koyama95} Koyama, K., et al., Nature, {\bf 378}, 255 (1995)

\bibitem{aha04} Aharonian, F.A., et al., Nature, {\bf 432}, 75 (2004)

\bibitem{pe98} Pohl, M.,Esposito, J.A., ApJ, {\bf 507}, 327 (1998)
 
\bibitem{ginzburg64} Ginzburg, V.L.\ \& Syrovatskii, S.I. (New York: Macmillan). (1964)
 
\bibitem{drury89} L.O'C.\ Drury, W.J.\ Markiewicz, H.J.\ V\"olk, A\& A, {\bf 225}, 179. (1989)

\bibitem{dunne} Dunne, B.C., Points, S.D., Chu, Y.H., ApJS, {\bf 136}, 119 (2001)

\bibitem{bamba04} Bamba, A., Ueno, M., Nakajima, H., Koyama, K., ApJ, {\bf 602}, 257. (2004)
 
%%%%%%%HERE%%%
\bibitem{bamba} Bamba, A., et al., ApJ\ {\bf 589}, 827. (2003)

\bibitem{vink} Vink, J., et al.,  ApJ\ {\bf 587}, L31--34. (2003)

\bibitem{kj05} Kang, H., Jones, T.W.,  ApJ {\bf 620}, 44. (2005)

\bibitem{be87} Blandford, R.D., Eichler, D., Phys. Rep. {\bf 154}, 1. (1987)

\bibitem{ab06} Amato, E., Blasi, P., MNRAS {\bf 371}, 1251. (2006)

\bibitem{vla06} Vladimirov, A., Ellison, D.C., Bykov, A., ApJ {\bf 652}, 1246. (2006)

\bibitem{drury83} Drury, L. O'C., Rep. Prog. Phys. {\bf 46}, 973. (1983)

\bibitem{wid02} Widrow, L.M.,  Rev. Mod. Phys. {\bf 74}, 775. (2002)

\bibitem{ss03} Schlickeiser, R., Shukla, P.K., ApJ {\bf 599}, L57. (2003)

\bibitem{med06} Medvedev, M.V., Silva, L.O., Kamionkowski, M., ApJ {\bf 642}, L1. (2006)

\bibitem{cc07} Cassam-Chena\"i, G., Hughes, J.P., Ballet, J., Decourchelle, A., ApJ {\bf 665}, 315. (2007)

\bibitem{bl} Bell, A.R., Lucek, S.G., MNRAS\ {\bf 321}, 433. (2001)

\bibitem{lb} Lucek, S.G., Bell, A.R., MNRAS\ {\bf 314}, 65. (2000)

\bibitem{bell04} Bell, A.R., MNRAS\ {\bf 353}, 550. (2004)

\bibitem{ply} M.~Pohl, H.~ Yan, A.~Lazarian,  ApJ\ {\bf 626}, L101-104. (2005)

\bibitem{voelk} H.J.~V\"olk, et al.,  A\& A\ {\bf 396}, 649--656. (2002)

\bibitem{ell07} D.C. Ellison, et al.,  ApJ {\bf 661}, 879--891. (2007)

\bibitem{bkv} E.G.~Berezhko, L.T.~Ksenofontov, H.J.~V\"olk,  A\& A\ {\bf 452}, 217. (2006)

\bibitem{cassam} G.~Cassam-Chena\"i, et al.,  A\& A\ {\bf 427}, 199.(2004)

\bibitem{hess-rx} F.~A.~Aharonian, et al.,  A\& A\ {\bf 464}, 235-243. (2007)

\bibitem{abdo} A.~A.~Abdo, et al.,  ApJ\ {\bf 658}, L33--36. (2007)

\bibitem{hunter} Hunter, S.D., et al.,  ApJ {\bf 481}, 205. (1997)
 
\bibitem{malvezzi} P. Picozza for the PAMELA Collaboration,  Astroparticle Physics {\bf 27}, 296–315 (2007)

\bibitem{andy04} Strong, A.W., Moskalenko, I.V., Reimer, O.,  ApJ {\bf 613}, 962 (2004)

\bibitem{buckley98} Buckley, J.H., et al.\  A\& A\ {\bf 329}, 639--658.(1998)

\bibitem{hess-rx6} Aharonian, F.A., et al.,  A\& A\ {\bf 449}, 223--242 (2006)

\bibitem{hess-vj} Aharonian, F.A., et al.,  A\& A\ {\bf 437}, L7--10 (2005)

\bibitem{kis+bea} Kistler, M.D., Beacom, J.F., PRD {\bf 74}, 063007 (2006)

\bibitem{hl80} Higdon, J.C., Lingenfelter, R.E.,  ApJ {\bf 239}, 867 (1980)

\bibitem{sp90} Spitzer Jr., L., ARA\& A {\bf 28}, 71 (1990)

\bibitem{hl06} Higdon, J.C., Lingenfelter, R.E., Adv. Spa. Res. {\bf 37}, 1913 (2006)

\bibitem{bru80} Bruhweiler, F.C., Gull, T.R., Kafatos, M., Sofia, S., ApJ {\bf 238}, L27 (1980)

\bibitem{par04} Parizot, E., et al.,  A\& A\ {\bf 424}, 747 (2004)

\bibitem{meyer} Meyer, J.P., Drury, L.O'C., Ellison, D.C.,  ApJ {\bf 487}, 182 (1997)

\bibitem{tw05} Tang, S., Wang, Q.D., ApJ {\bf 628}, 205--209. (2005)

\bibitem{anch} Anchordoqui, L.A., et al.,  PRL {\bf 98}, 121101. (2007)

\bibitem{binns} Binns, R., et al.,  ApJ {\bf 634}, 351 (2005)

\bibitem{mccg02} McClure-Griffiths, N.M., Dickey, J.M., Gaensler, B.M., Green, A.J., ApJ {\bf 578}, 176 (2002)

\bibitem{cesarsky83} Cesarsky, C.J., Montmerle, T., Space Science Reviews {\bf 36}, 173--193. (1983)
 
\bibitem{bykov01} Bykov, A.M., Space Science Reviews {\bf 99}, 317-326. (2001)

\bibitem{reimer} Aharonian, F., et al.,  A\& A\ {\bf 467}, 1075. (2007)

\bibitem{hess-survey} Aharonian, F., et al.,  ApJ\ {\bf 636}, 777--797 (2006)

\bibitem{drury94} Drury, L.O'C.,\ Aharonian, F.A.,\ V\"olk, H.J., A\& A\ {\bf 287}, 959-971. (2004)

\bibitem{rothenflug04} Rothenflug, R., et al.\  A\& A\ {\bf 425}, 121-131. (2004)

\bibitem{rho01} Rho, J.,\ Jarrett, T.H.,\ Cutri, R.M.,\ Reach, W.T.,  ApJ\ {\bf 547}, 885-898. (2001)

\bibitem{huang} Huang, C.-Y.,. Park, S.-E., Pohl, M., Daniels, C., Astropart. Phys. {\bf 27}, 429. (2007)

\bibitem{kieda2001} Kieda, D.B. Swordy, S.P., Wakely, S.P., Astropart. Phys. {\bf 15}, 287 (2001)

\bibitem{hess-direct} Aharonian, F., et al.,  PRD\ {\bf 75}, 042004. (2007)



%{END REFERENCES FOR SNR}

% BEGIN GCO

\bibitem{DeJager06} De Jager, O.C.\ , in ``Astrophysical Sources of
High Energy Particles and Radiation'',  held in Torun, Poland, eds. T.\
Bulik, B. Rudak, and G. Madejski, p.\ 298. (2006)

\bibitem{Aharonian05} Aharonian, F. et al. [HESS Collaboration],  A
\& A {\bf 435}, L17. (2005)

\bibitem{Aharonian06} Aharonian, F. et al. ,  A\&A, {\bf 448}, L43. (2006)

\bibitem{Blondin01} Blondin, J.M., Chevalier, R.A., Frierson, D.M.\
, Astrophys. J.\ {\bf 563}, 806-815. (2001)

\bibitem{hess1804} Aharonian, F.\ et al.\ , Science {\bf 307}, 1938. (2005)

\bibitem{hess1825} Aharonian, F.\ et al.\ , Astron.\ Astrophys.\ {\bf 442}, L25-L29. (2006)

\bibitem{hess1718} Aharonian, F.\ et al.\ , Astron.\ Astrophys.\ {\bf 472}, 489-495. (2007)

\bibitem{hessVelax} Aharonian, F.\  et al.\ , Astron.\ Astrophys.\ {\bf 448}, L43-L47. (2006)

\bibitem{Funk06} Funk, S.\ , Astrophys. Space Sci.\ to appear, arXiv:astro-ph/0609586. (2006)

\bibitem{Thompson04} Thompson, D. J.\ , ed. K. S. Cheng \& G. E. Romero  (Kluwer), ApSS, {\bf 304} , 149. (2004)

\bibitem{Daugherty96} Daugherty, J. K. \& Harding, A. K. , ApJ,{\bf  458}, 278. (1996)

\bibitem{Romani96} Romani, R. W. , ApJ, {\bf 470}, 469. (1996)

\bibitem{Lessard00} Lessard, R.W.\ et al.\ , Astrophys.\ J.\ {\bf 531}, 942-948. (2000)

\bibitem{magic_psr1951} Albert, J.\ et al.\ , Astrophys.\ J.\, in press. (2007)

\bibitem{Hirotani07} Hirotani,  ApJ {\bf 662}, 1173 (2007)

\bibitem{Harding05} Harding, A.K., Usov, V.V., Muslimov, A.G.\ , ApJ, {\bf 622}, 531. (2005)

\bibitem{Mirabel06} Mirabel, F.\ , Science, {\bf 312}, 1759-1760.  (2006)

\bibitem{Corbel02} Corbel, S.\ et al.\ , Science{\bf  298}, 196-199. (2002)

\bibitem{Kaaret03} Kaaret, P.\ et al.\ , Astrophys.\ J.\ {\bf 582}, 945-953. (2003)

\bibitem{hess1259} Aharonian, F.A.\ et al.\ , Astro.\ Astrophys.{\bf  442}, 1-10. (2005)

\bibitem{magic_ls61} Albert, J.\ et al.\ , Science, {\bf 312}, 1771-1773.  (2006)

\bibitem{magic_cygx1} Albert, J.\ et al.\ , Astrophys.\ J.{\bf  665}, L51-L54. (2007)

\bibitem{Tavani96} Tavani, M.\ et al.\ , Astron.\ Astrophys.\ Suppl.\ {\bf 120}, 221-226. (1996)

\bibitem{Casares05} J.\ Casares et al.\ , MNRAS{\bf 360}, 1091-1104. (2005)

\bibitem{Leahy97} Leahy, D. et al.:ApJ {\bf 475}, 823 (1997)

\bibitem{Taylor96} Taylor, G. et al.: A$\&$A {\bf 305}, 417 (1996)

\bibitem{Massi01} Massi, M. et al.: ApJ {\bf 376}, 217 (2001)

\bibitem{Dhawan06} Dhawan, V. et al: Proceedings of VI Microquasar Workshop, in press (2006)

\bibitem{hess_ls5039} Aharonian, F.\ , Science {\bf 309},746-749. (2005)

\bibitem{Paredes00} Paredes, J.M.\ et al.\ , Science {\bf 288}, 2340-2342. (2000)

\bibitem{Bosch05} Bosch-Ramon, V.\ et al.\ , Astrophys.\ J.\ {\bf 628}, 388-394. (2005)

\bibitem{Torres06} Torres, D.F.\ \& Halzen, F.\ , arXiv:astro-ph/0607368 (2006)

\bibitem{Fender03} Fender, R.P., Gallo, E., Jonker, P.G.\ , Mon.\ Not.\ Roy.\ Astronom.\ Soc.\ {\bf 343}, L99-L103. (2003)

\bibitem{Gallo05} Gallo, E.\ et al.\ , Nature {\bf 436}, 819-821. (2005)

\bibitem{Corbel00} Corbel, S.\ et al.\ , Astron.\ Astrophys.\ {\bf 359}, 251-268. (2000)

%{END REFERENCES FOR GCO}

% References dark matter

\bibitem{Spergel:2006hy}
  Spergel, D.N., {\it et al.}  [WMAP Collaboration],
  %``Wilkinson Microwave Anisotropy Probe (WMAP) three year results:
  %Implications for cosmology,''
  Astrophys.\ J.\ Suppl.\  {\bf 170}, 377 (2007).


%\cite{Percival:2006gt}
\bibitem{Percival:2006gt}
  Percival, W.J.,  { et al.},
  %``The shape of the SDSS DR5 galaxy power spectrum,''
  Astrophys.\ J.\  {\bf 657}, 645 (2007)
 % [arXiv:astro-ph/0608636].
  %%CITATION = ASJOA,657,645;%%

% { JB4 {
\bibitem{baltz_p5_06} Baltz, E.A., P5 presentation (2006)
% } JB4

\bibitem{Zwicky1933} Zwicky, F., Helvetica Physica Acta\ {\bf 6}, 110--127 (1933).

\bibitem{CowsikMcClelland(1973)} Cowsik, R., McClelland, J., \apj, {\bf 180}, 7 (1973).

% Proof of dark matter.
\bibitem{clowe06} Clowe, D., et al., \apjl, {\bf 648}, (2006) L109. 

% JB3 {
\bibitem{baltz06} Baltz, E.A., et al.,
Phys. Rev. D., {\bf 74}, 103521 (2006)

\bibitem{aprile05} Aprile, E., et al., New Astron. Rev., {\bf 49}, 289 (2005)

\bibitem{klapdor05} Klapdor-Kleingrothaus, H.V., Krivosheina, I.V., Nucl.
Phys. B. (Proc. Suppl.), {\bf 145}, 237 (2005).

\bibitem{klapdor02} Klapdor-Kleingrothaus, H.V., et al., Nucl. Inst. and
Methods Phys. Res. A, {\bf 481}, 149 (2002).

\bibitem{bisset07} Bisset, R., et al., Nucl. Phys. B. (Proc. Suppl.), {\bf 173},
164 (2007).

\bibitem{akerib05} Akerib, D.S., et al., Nucl. Inst. and Methods Phys. Res. A, {\bf 559}, 411 (2005).

\bibitem{morales99} Morales, A., TAUP99, Paris (1999).

\bibitem{sanglard07} Sanglard, V., et al., Nucl. Phys. B. (Proc. Suppl.),
{\bf 173}, 99.

\bibitem{ibarratran08} Ibarra, A., Tran, D., Phys. Rev. Lett., {\bf 100},
061301 (2008)
% } JB3

% \bibitem{machos} C.~Alcock, et~al., Astrophys. J. {\bf 550}, L169 (2001).

% \bibitem{bekenstein} J.D.~Bekenstein, Contemp. Phys. {\bf 46}, 387 (2006).

\bibitem{bergstrom06} Bergstr\"om, L., et al., arXiv:astro-ph/0609510v1 (2006).

% \bibitem{tevscale???}
\bibitem{amelino98} Amelino-Camelia, G., et~al., Nature, {\bf 393}, 319 (1998)

\bibitem{biller99} Biller, S.D., et~al., Phys.~Rev.~Lett., {\bf 83}, 2108 (1999)

% JB4 {
\bibitem{birkedal06} ABirkedal, A., et al., 
Phys.~Rev.~D., {\bf 74}, 035002 (2006).
% }

\bibitem{kraussnasri} Krauss, L.M., Nasri, S., Trodden, M., Phys. Rev. D, {\bf 67}, 085002 (2003).

\bibitem{zee80} Zee, A., Phys. Lett., {\bf B93}, 339 (1980);
Phys. Lett., {\bf B161}, 141 (1985).

\bibitem{baltzbergstrom} Baltz, E.A., and Bergstr\"om, L., Phys. Rev. D
{\bf 67}, 043516 (2003).

\bibitem{bringmann07} Bringmann, T., Bergstr\"om, L., Edsj\"o, J.,
arXiv:hep-ph/0710.3169v1 (2007).

% JB3 {
\bibitem{ferrer06} Ferrer, F., Krauss, L.M., Profumo, S., Phys. Rev. D.,
{\bf 74}, 115007 (2006)
% } JB3

\bibitem{nfw97} Navarro, J.~F., Frenk, 
C.~S., \& White, S.~D.~M. \apj, {\bf 490}, 493 (1997).

\bibitem{moore99} Moore, B., Quinn, T., 
Governato, F., Stadel, J., \& Lake, G.\, \mnras, {\bf 310}, 1147  (1999).

\bibitem{Netal} Navarro, J.F., et~al., MNRAS, {\bf 349},
1039 (2004).

\bibitem{DZMSC} Diemand, J., et~al., MNRAS, {\bf 364}, 665
(2005).

\bibitem{SKBK06} Strigari, L.E., et al., 
astro-ph/0611925 (2006).

\bibitem{bub98} Bergstr{\"o}m, L., Ullio, P., Buckley, J.H., Astroparticle Physics, {\bf 9}, 137 (1998).

\bibitem{kosack04} Kosack, K., { et al.}, \apjl, {\bf 608}, L97 (2004).

\bibitem{GCHESS2004} Aharonian, F., { et~al.}, \aap {\bf 425}, L13--L17 (2004).

\bibitem{Horns2005} Horns, D., Physics Letters B, {\bf 607}, 225--232 (2005).

\bibitem{Profumo:2005xd} Profumo, S., Phys. Rev. D, {\bf 72}, 103521 (2005).

%\cite{Stoehr:2003hf}
\bibitem{Stoehr:2003hf}
  Stoehr, F., et al.,
  %``Dark matter annihilation in the Milky Way's halo,''
  MNRAS {\bf 345}, 1313 (2003)
 % [arXiv:astro-ph/0307026].
  %%CITATION = MNRAA,345,1313;%%

%JB3 {
\bibitem{serpico08}
P.D.~Serpico and G.~Zaharijas, 2008arXiv0802.3245S (2008)
% } JB3

%\cite{Diemand:2006ik}
\bibitem{Diemand:2006ik}
  Diemand, J., Kuhlen, M., Madau, P., 
  %``Dark matter substructure and gamma-ray annihilation in the Milky Way
  %halo,''
  Astrophys.\ J.\  {\bf 657}, 262 (2007)
 % [arXiv:astro-ph/0611370].
  %%CITATION = ASJOA,657,262;%%

\bibitem{fornengo04} Fornengo, N., Pieri, L., Scopel, S.,  Phys. Rev. D.,
{\bf 70}, 103529 (2004).


\bibitem{Vassiliev2003} Vassiliev, V.V., 
%Search for TeV Annihilation Radiation from Supersymmetric Dark Matter in nearby Galaxies}},
28th Int. Cosmic Ray Conf.(Tsukuba), 2679-2682 (2003).

\bibitem{LeBohec2003} LeBohec, S. L.,  \& VERITAS Collaboration,
%\newblock \bibinfo{title}{{Search for a WIMP Annihilation Signature in the Core
  %of the Globular Cluster M15}}.
28th Int. Cosmic Ray Conf. (Tsukuba), 2521-2524 (2003).

\bibitem{woodetal07} Wood, M., et~al., submitted (2007).

% JB3 {
\bibitem{moulin07} Aharonian, F., et~al., Astropart.~Phys., {\bf 29}, 55 (2008).
% } JB3

\bibitem{Betal02} Baltz, E., et~al., Phys. Rev. D, {\bf 61}, 023514 (2000).

\bibitem{Tyler02} Tyler, C., Phys. Rev. D, {\bf 66}, 023509 (2002).

\bibitem{EFS04} Evans, N.W., Ferrer, F., Sarkar, S., Phys. Rev. D, {\bf 69},
123501 (2004).

\bibitem{BH06} Bergstr\"om, L., Hooper, D., Phys. Rev. D, {\bf 73}, 063510 (2006).

\bibitem{PB04} Pieri, L., Branchini, E., Phys. Rev. D, {\bf 69}, 043512 (2006).

\bibitem{Strigari:2007at}
  Strigari, L.E., et al.
  %``The Most Dark Matter Dominated Galaxies: Predicted Gamma-ray Signals from
  %the Faintest Milky Way Dwarfs,''
  arXiv:0709.1510 [astro-ph].
  %%CITATION = ARXIV:0709.1510;%%

% JB3 { From FF
\bibitem{belokurov} Belokurov, V.,  et al., Astrophys.~J., {\bf 654}, 897 (2007).
% } JB3

% JB4 {
\bibitem{martin07} Martin, N.F., et al., MNRAS, {\bf 380}, 281 (2007).
% } JB4

% JB3 { From FF
\bibitem{metz} Metz, M., Kroupa, P.,  MNRAS, {\bf 376}, 387 (2007).

\bibitem{munoz07} Munoz, R.R., Majewski, S.R., Johnston, K.V., arXiv:0712.4312v1 [astro-ph] (2007).
% } JB3

\bibitem{Klypin:1999uc} Klypin, A., et al., 
Astrophys. J. {\bf 522}, 82 (1999).

\bibitem{Moore:1999wf} Moore, B., et~al., Astrophys. J., {\bf 524}, L19 (1999).

\bibitem{1992ApJ...398...43C} Carlson, E.D., Machacek, M.E., Hall, L.J., 
Astrophys. J., {\bf 398}, 43 (1992).

\bibitem{Spergel:1999mh} Spergel, D.N., Steinhardt, P.J., Phys. Rev. Lett.,
{\bf 84}, 3760 (2000).

\bibitem{Kaplinghat:2000vt} Kaplinghat, M., Konx, L., Turner, M.S., Phys. Rev.
Lett., {\bf 85}, 3335, (2000).

\bibitem{Kamionkowski:1999vp} Kamionkowski, M., Liddle, A.R.,  Phys. Rev. Lett.,
{\bf 84}, 4525 (2000).

\bibitem{Zentner:2002xt} Zentner, A.R., Bullock, J.S., Phys. Rev. {\bf D66},
043003, (2002).

\bibitem{1986ApJ...303...39D} Dekel, A., Silk, J., Astrophys. J., {\bf 303}, 39
(1986).

\bibitem{1999ApJ...523...54B} Barkana, R., Loeb, A., Astrophys. J., {\bf 523},
 54, (1999).

\bibitem{2001ApJ...548...33B} Bullock, J.S., Kravtsov, A.V., Weinberg, D.H., 
Astrophys. J., {\bf 548}, 33, (2001).

\bibitem{Koushiappas:2003bn} Koushiappas, S.M., Zentner, A.R., Walker, T.P., 
Phys. Rev., {\bf D69}, 043501, (2004).

\bibitem{Setal99} Schmid, C., et~al., Phys. Rev. D, {\bf 59}, 043517 (1999).

\bibitem{Hetal01} Hofmann, S., et~al., Phys. Rev. D, {\bf 64}, 083507 (2001).

\bibitem{Chenetal01} Chen, X., et~al., Phys. Rev. D, {\bf 64}, 021302 (2001).

\bibitem{Berezinskyetal03} Berezinsky, V., et~al., Phys. Rev. D, {\bf 68},
103003 (2003).

\bibitem{Green04} Green, A.M., Hofmann, S., Schwarz, D.J., MNRAS, {\bf 353}, L23 (2004).

\bibitem{Green05} Green, A.M., et~al., J. Cosmol. Astropart. Phys., {\bf 08},
003, (2005).

\bibitem{LZ05} Loeb, A., Zaldarriaga, M., Phys. Rev. D, {\bf 71}, 103520 (2005).

\bibitem{Bertch} Bertschinger, E., Phys. Rev. D, {\bf 74}, 063509 (2006).

\bibitem{Mooreetal06} Moore, B., et~al., astro-ph/0502213

\bibitem{K06} Koushiappas, S.M., Phys. Rev. Lett., 97, 191301 (2006).

\bibitem{peebles:1972} Peebles, P. J. E.,  Astrophys.\ J.\, {\bf 178}, 371 (1972).

\bibitem{young:1980}
  Young, P., Astrophys.\ J.\ {\bf 242}, 1232 (1980).

%\cite{Ipser:1987ru}
\bibitem{Ipser:1987ru}
  Ipser, J.R., Sikivie, P.,
  %``Estimates Of The Density Of Dark Matter Near The Center Of The Galaxy,''
  Phys.\ Rev.\ D {\bf 35}, 3695 (1997).
  %%CITATION = PHRVA,D35,3695;%%

\bibitem{Quinlan:1995}
  Quinlan, G.D., Hernquist, L., Sigurdsson, S.,
  Astrophys.\ J.\  {\bf 440}, 554 (1995).

\bibitem{Gondolo:1999ef}
  Gondolo, P., Silk, J., 
  %``Dark matter annihilation at the galactic center,''
  Phys.\ Rev.\ Lett.\  {\bf 83} 1719 (1999)
 % [arXiv:astro-ph/9906391].
  %%CITATION = ASTRO-PH 9906391;%%

% WMAP results
\bibitem{Merritt:2003qc}
  Merritt, D.,
  %``Single and Binary Black Holes and their Influence on Nuclear Structure,''
  Proceedings of Carnegie Observatories Centennial Symposium
  % { Coevolution of Black Holes and Galaxies}
  [arXiv:astro-ph/0301257].
  %%CITATION = ASTRO-PH 0301257;%%

%\cite{Bertone:2005hw}
\bibitem{Bertone:2005hw}
  Bertone, G., Merritt, D.,
  %``Time-dependent models for dark matter at the Galactic center,''
  Phys.\ Rev.\ D {\bf 72}, 103502 (2005)
 % [arXiv:astro-ph/0501555].
  %%CITATION = ASTRO-PH 0501555;%%

%\cite{Bertone:2005hw,Bertone:2005xv}
\bibitem{Bertone:2005xv}
  Bertone, G., Merritt, D.,
  %``Dark matter dynamics and indirect detection,''
  Mod.\ Phys.\ Lett.\ A {\bf 20}, 1021 (2005)
 % [arXiv:astro-ph/0504422].
  %%CITATION = ASTRO-PH 0504422;%%


\bibitem{Ullio:2001fb}
  Ullio, P., Zhao, H.,  M.~Kamionkowski, M.,
  %``A Dark-Matter Spike at the Galactic Center?,''
  Phys.\ Rev.\ D {\bf 64}, 043504 (2001)
 % [arXiv:astro-ph/0101481].
  %%CITATION = ASTRO-PH 0101481;%%

\bibitem{Merritt:2002vj}
  Merritt, D., Milosavljevic, M., Verde, L., Jimenez, R.,
  %``Dark matter spikes and annihilation radiation from the galactic center,''
  arXiv:astro-ph/0201376.
  %%CITATION = ASTRO-PH 0201376;%%

%\cite{Merritt:2003eu,Bertone:2005hw}
\bibitem{Merritt:2003eu}
  Merritt, D., 
  %``Dark matter spikes and indirect detection,''
  arXiv:astro-ph/0301365.
  %%CITATION = ASTRO-PH 0301365;%%
% } JB 10/1/07 added from Bertone


\bibitem{Madau:2001}
  Madau, P., Rees,M.J., Astrophys.\ J.\ Lett.\, {\bf 551}, L27 (2001).

\bibitem{Bertone:2005xz}
  Bertone, G., Zentner, A.R., Silk, J.,
  %``A new signature of dark matter annihilations: Gamma-rays from intermediate-mass black holes,''
  Phys.\ Rev.\ D {\bf 72}, 103517  (2005).
  %%CITATION = ASTRO-PH 0509565;%%

%\cite{Zhao:2005zr}
\bibitem{Zhao:2005zr}
  Zhao, H.S., Silk, J.,
  %``Mini-dark halos with intermediate mass black holes,''
  arXiv:astro-ph/0501625.
  %%CITATION = ASTRO-PH 0501625;%%

\bibitem{islamc:2004}
  Islam, R., Taylor, J., Silk, J.,
  MNRAS {\bf 354}, 443 (2003).

\bibitem{islamb:2004}
  Islam, R., Taylor, J., Silk, J.,
  MNRAS {\bf 354}, 427 (2004).

%\cite{Koushiappas:2003zn}
\bibitem{Koushiappas:2003zn}
  Koushiappas, S.M., Bullock, J.S., Dekel, A.,
  %``Massive black hole seeds from low angular momentum material,''
  MNRAS\  {\bf 354}, 292 (2004)
%  [arXiv:astro-ph/0311487].
  %%CITATION = ASTRO-PH 0311487;%%

\bibitem{JE2004} Edsj{\"o}, J., Schelke, M., Ullio, P.,
%\newblock \bibinfo{title}{{Direct versus indirect detection in mSUGRA with
  %self-consistent halo models}},
Journal of Cosmology and Astro-Particle Physics, {\bf 009}, 004-1--004-25
  (2004).

\bibitem{BG2002} Baltz, E.A., Gondolo, P.,
%\newblock \bibinfo{title}{{Improved constraints on supersymmetric dark matter
  %from muon g-2}},
{\prd}, {\bf 67}, 063503-1--063503-8 (2003).

\bibitem{Bottino2003} Bottino, A., Donato, F., Fornengo, N., Scopel, S.,
%\newblock \bibinfo{title}{{Lower bound on the neutralino mass from new data on
  %CMB and implications for relic neutralinos}},
{\prd}, {\bf 68}, 043506-1 (2003)

\bibitem{Bottino2004} Bottino, A., Donato, F., Fornengo, N., Scopel, S.,
%\newblock \bibinfo{title}{{Light neutralinos and WIMP direct searches}},
{\prd}, {\bf 69}, 037302-1 (2004)

\bibitem{GK1990} Griest, K., Kamionkowski, M.,
%\newblock \bibinfo{title}{{Unitarity limits on the mass and radius of
  %dark-matter particles}},
{\prl}, {\bf 64}, 615 (1990).

\bibitem{profumo05}  Profumo, S., \prd, {\bf 72}, 
103521 (2005).

\bibitem{tsuchiya04} Tsuchiya, K., Enomoto, R., Ksenofontov, L. T., et al., ApJ 606, L115 (2004)..

\bibitem{koushiappas_santafe06} Koushiappas, S., talk at
"Ground-based Gamma-ray Astronomy: Towards the Future, May 11-12, Santa Fe (2006).


%{END REFERENCES FOR DARK MATTER}

%{BEGIN REFERENCES FOR ESWG02}

\bibitem{Sreekumar1999} Sreekumar, P., Bertsch, D.~L., Hartman, R.~C., Nolan, P.~L. and Thompson, D.~J., Astroparticle Phys., {\bf 11},
221 (1999).

\bibitem{Aharonian2007M87} Aharonian, F. Akhperjanian, A.~G., Bazer-Bachi, A.~R., et al., Science {\bf 314}, 1424 (2006)

\bibitem{Tavecchio2005} Tavecchio, F., The Tenth Marcel Grossmann Meeting.~ , 512 (2005)

\bibitem{Krawczynski2006} Krawczynski, H., Astronomical Society of the Pacific Conference Series, {\bf 350}, 105 (2006)

\bibitem{Hartman1999} Hartman, R.~C., et al., \apjs, {\bf 123}, 79 (1999)

\bibitem{Punch1992} Punch, M., et al., \nat, {\bf 358}, 477 (1992)

%\bibitem{Foss:04} Fossati, G., Buckley, J., Edelson, R.~A., 
%Horns, D., \& Jordan, M.\ 2004, New Astronomy Review, 48, 419 

\bibitem{Foss:08} {Fossati, G., et al., \apjl, {\bf 677}, L2 (2008)}

\bibitem{Aharonian2005} Aharonian, F., et al., \aap, {\bf 441}, 465 (2005)

\bibitem{Horan2004} Horan, D., \& Weekes, T.~C., New Astronomy Review, {\bf 48}, 527 (2004)

\bibitem{Stec:92} {Stecker, F.\ W., De Jager, O.\ C.,  \& Salamon, M.~H.,\apj, {\bf 390}, L49 (1992)}

\bibitem{1996Natur.383..319G} Gaidos, J.~A., et al., \nat, {\bf 383}, 319 (1996)

\bibitem{1996ApJ...472L...9B} Buckley, J.~H., et al., \apjl, {\bf 472}, L9 (1996)

\bibitem{1996ApJ...470L..89T} Takahashi, T., et al., \apjl, {\bf 470}, L89 (1996)

\bibitem{Unwi:02}{Unwin, S.C., Wehrle, A.E., Jones, D.L., Meier, D.L., and Piner, B.G.,  
Publ. of the Astronomical Society of Australia, {\bf 19}, 5 (2002)}

\bibitem {Grin:05}{Grindlay, J.E., New Astron.Rev., {\bf 49}, 436 (2005)}

\bibitem{2000A&A...353...97K} Krawczynski, H., Coppi, P.~S., Maccarone, T., \& Aharonian, F.~A., \aap, {\bf 353}, 97  (2000)

\bibitem{2006ApJ...653L...5G} Georganopoulos, M., Perlman, E.~S., Kazanas, D., \& McEnery, J., \apjl, {\bf 653}, L5 (2006)

\bibitem{Blandford1976} Blandford, R.~D., \mnras, {\bf 176}, 465 (1976)

\bibitem{Blandford1977} Blandford, R.~D., \& Znajek, R.~L., \mnras, {\bf 179}, 433 (1997)

\bibitem{Lovelace1976} Lovelace, R.~V.~E., \nat, {\bf 262}, 649 (1976)

\bibitem{Levinson2000} Levinson, A., Physical Review Letters, {\bf 85}, 912 (2000)

\bibitem{2007ApJ...659.1063K} Krawczynski, H., \apj, {\bf 659}, 1063 (2007)

\bibitem{Roma:97} Romanova, M.~M., \& Lovelace, R.~V.~E.\ 1997, \apj, {\bf 475}, 97 (1997)

\bibitem{Kund:04}{ Kundt, W., Gopal, K., JApA, {\bf 25}, 115 (2004)}

\bibitem{deYo:06}{De Young, D., ApJ, {\bf 648}, 200 (2006)}

\bibitem{Nogu:07}{Noguchi, K., \& Liang, E., Astrophys. \& Space Sci., {\bf 307}, 315 (2007)}

\bibitem{Nish:07} {Nishikawa, K.-I., Hededal, C.B., Hardee, P.E., Fishman, G.J.,Kouveliotou, C., \& Mizuno, Y., Astrophys. \& Space Sci., {\bf 307}, 319, (2007)}

\bibitem{Love:05}{Lovelace, R.V.E., Gandhi, P.R., \& Romanova, M.M., Astrophys. \& Space Sci., {\bf 298}, 115 (2005)}

\bibitem{Chan:07}{Chang, P., Spitkovsky, A., \& Arons, J., ApJ, in press (arXiv:0704.3832v1) (2008)}

\bibitem{Aharonian2000} Aharonian, F.~A.\ 2000, New A, {\bf 5}, 377 (2000)

\bibitem{Muecke2001} M{\"u}cke, A., \& Protheroe, R.~J.\, Astroparticle Physics, {\bf 15}, 121 (2001)

\bibitem{Muecke2003} M{\"u}cke, A., Protheroe, R.~J., Engel, R., Rachen, J.~P., \& Stanev, T., Astroparticle Physics, {\bf 18}, 593 (2003)

\bibitem{Mannheim1993} Mannheim, K., \aap, {\bf 269}, 67  (1993)

\bibitem{Lovelace1979} Lovelace, R.~V.~E., MacAuslan, J., \& Burns, M., AIP Conf.~Proc.~56: Particle 
Acceleration Mech. in Astrophys., {\bf 56}, 399 (1979)

\bibitem{Burns1982} Burns, M.~L., \& Lovelace, R.~V.~E., \apj, {\bf 262}, 87 (1982)

\bibitem {Blandford1995} Blandford, R.~D., \& Levinson, A., \apj, {\bf 441}, 79 (1995)

\bibitem{Levinson1995} Levinson, A., \& Blandford, R., \apj, {\bf 449}, 86 (1995)

\bibitem {Halz:05} Halzen, F., Hooper, D., Astropart.Phys., {\bf 23}, 537 (2005)
 %% EGS_GRBs %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% EGS_CRs %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{SMR2000} Strong, A., Moskalenko, I.~V. \& Reimer, O., Proc. 26th Int. Cosmic Ray Conf. (Salt Lake), {\bf 4}, 52 (1999).

\bibitem{DiffGC2006} Aharonian, F. et~al. \nat {\bf 439}, 695 (2006).

\bibitem{Sreekumar1992} Sreekumar, P. et~al., \apj {\bf 400} L67 (1992).

\bibitem{Volk1996} Volk, H.~J., Aharonian, F.~A. \& Breitschwerdt, D., Space Science Reviews {\bf 75}, 279 (1996).

\bibitem{Pohl1994} Pohl, M., \aap, {\bf 287}, 453 (1994).

\bibitem{Nagai2005} Nagai, T., Search for TeV Gamma-Ray Emission from Nearby Starburst Galaxies (Ph.D.~Thesis), UMI Publishing (2005).

\bibitem{Gotting2005} Gotting, N., Ph.D.~Thesis (2006)

\bibitem{Itoh2002} Itoh, C., et~al., \aap {\bf 396}, L1 (2002).

\bibitem{HESS253} Aharonian, F. et~al. \aap, {\bf 442}, 177 (2005).

\bibitem{Torres2004} Torres, D.~F., Reimer, O., Domingo-Santamar{\'{\i}}a, E. \& Digel, S.~W.,
\apjl, {\bf 607}, L99 (2004).

\bibitem{Torres2004a} Torres, D.~F., \apj, {\bf 617}, 966 (2004).

\bibitem{VoelkAtoyan1999} V{\"o}lk, H.~J., Atoyan, A.~M., Astroparticle Physics,{\bf 11}, 73 (1999),

\bibitem{EnsslinBiermann1998} Ensslin, T.~A. \& Biermann, P.~L., \aap,{\bf 330}, 90 (1998).

\bibitem{Keshet2002} Keshet, U., Waxman, E., Loeb, A., Springel, V. \& Hernquist, L., \apj,{\bf 585}, 128 (2003).

\bibitem{GB2003} Gabici, S. \& Blasi, P., Astroparticle Physics, {\bf 20}, 579 (2004)

\bibitem{Perkins2006} Perkins, J.~S. et~al. \apj, {\bf 644}, 148, 2006

\bibitem{HessCluster}{W. Domainko, W. Benbow, J. A. Hinton, et al., Contrib. to the 30th ICRC, Merida, Mexico [arXiv:0708.1384] (2007)}

\bibitem{Volk2003} Voelk, H.~J., arXiv:astro-ph/0303078 (2003).

\bibitem{BD2004} Berrington, R.~C. \& Dermer, C.~D. arXiv:astro-ph/0407278 (2004)

\bibitem{R2004} Reimer, A., Reimer, O., Schlickeiser, R. \& Iyudin, A., \aap, {\bf 424} 773, (2004)

\bibitem{Rf2004} Rordorf, C., Grasso, D. \& Dolag, K., Astroparticle Physics, {\bf 22}, 167 (2004)

\bibitem{2003MNRAS.342.1009M} Miniati, F.\, \mnras, {\bf 342}, 1009 (2003)

\bibitem{Elew:06}{V. Van Elewyck, Proc. Int. School of Cosmic Ray Astrophysics, 15th Course, Erice, Italy, astro-ph/0612731 (2006)}

\bibitem {2005PhRvL..95y1102G} Gabici, S., \& Aharonian, F.~A., Physical Review Letters, {\bf 95}, 251102 (2005)

\bibitem{ad07} {Atoyan, A., and Dermer, C., \apj (in preparation) (2007)}

\bibitem{2007ApJ...664L..71A} Aharonian, F., et al., ApJL, 664, L71 (2007)

\bibitem{2001ApJ...559..187K} Krawczynski, H., et al., ApJ, 559, 187 (2001)

\bibitem{2008MNRAS.384L..19B} Begelman, M.~C., Fabian, A.~C., and {Rees}, M.~J., MNRAS, 384, 
L19 (2008)

\bibitem{2008ApJ...677..906F} Fossati, G., et al., ApJ, 677, 906 (2008)

\bibitem{2008Natur.452..966M} Marscher, A.~P., et al., Nature, 452, 966 (2008)

\bibitem{2008arXiv0804.3096S} Spruit, H.~C., ArXiv e-prints, 0804.3096 (2008)
 
\bibitem{2007arXiv0709.1475T} Teshima, M., et al., ArXiv e-prints, 0709.1475 (2007)


%% EGS_EBL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem {Goul:67} Gould, R. J., \& Schr\` eder, G., Phys. Rev., {\bf 155}, 1408M (1967)
\bibitem {Haus:01} Hauser, M.G., \& Dwek, E., ARA \& A, {\bf 39}, 249 (2001)
\bibitem {Bill:95} Biller, S.D. et.al., ApJ, {\bf 445}, 227 (1995)
\bibitem {Vass:99} Vassiliev, V.V., Astroppart. Phys., {\bf 12}, 217 (2000)
\bibitem {Dwek:05} Dwek, E., Krennrich, F.  \& Arendt, R., ApJ {\bf 634}, 155 (2005)
\bibitem {Ahar:06} Aharonian, F., et al., Nature, {\bf 440}, 1018 (2006)
\bibitem {Mazi:07} Mazin, D., \& Raue, M., astro-ph/0701694 (2007)
\bibitem {Copp:99} Coppi, P.~S., \& Aharonian, F.~A.\ 1999, Astroparticle Physics, {\bf 11}, 35 (1999)
\bibitem {Kren:02} Krennrich, F. et al, \apj, {\bf 579}, L9 (2002)
\bibitem {Ahar:02} Aharonian, F., et al., A\&A, {\bf 393}, 89 (2002)
\bibitem {Ahar:94} Aharonian, F.~A., Coppi, P.~S., \& Voelk, H.~J., \apjl, {\bf 423}, L5  (1994)
%% AP_ DM %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Spergel2006} Spergel, D.~N., et~al., astro-ph/0603449 (2006).

\bibitem{EPP2010} EPP2010 Report:, \url{http://www7. nationalacademies.org/bpa/EPP2010.html} (2006)




\bibitem{Ju1996}
{{Jungman}, G.}, {{Kamionkowski}, M.} \&
  {{Griest}, K.}
 {\physrep} {\bf 267},
  195 (1996).

\bibitem{Sj2001}
{{Sj{\"o}strand}, T.} \emph{et~al.}
 {Computer Physics Communications}
  {\bf 135}, 238
  (2001).

\bibitem{DarkSUSY}
{{Gondolo}, P.} \emph{et~al.}
 {Journal of Cosmology and Astro-Particle
  Physics} {\bf 7}, 008-1
  (2004).

\bibitem{BEG2005}
{{Bergstr{\"o}m}, L.}, {{Bringmann}, T.},
  {{Eriksson}, M.} \& {{Gustafsson}, M.}
 {\prl}
  {\bf 94}, 131301-1
  (2005).

\bibitem{EM2005}
{{Els{\"a}sser}, D.} \& {{Mannheim}, K.}
 {\prl}
  {\bf 94}, 171302-1
  (2005), 

\bibitem{deB2006}
{{de Boer}, W.}, {{Sander}, C.},
  {{Zhukov}, V.}, {{Gladyshev}, A.~V.} \&
  {{Kazakov}, D.~I.}
 {\prl}
  {\bf 95}, 209001-1
  (2005).


\bibitem{GMMDT2006}
{{Graham}, A.~W.}, {{Merritt}, D.},
  {{Moore}, B.}, {{Diemand}, J.} \&
  {{Terzic}, B.}
 {astro-ph/0608613}
  (2006)

\bibitem{DMS2005}
{{Diemand}, J.}, {{Moore}, B.} \&
  {{Stadel}, J.}, {\nat}, {\bf 433}, 389 (2005).

\bibitem{GGMDS2006}
{{Goerdt}, T.}, {{Gnedin}, O.~Y.},
  {{Moore}, B.}, {{Diemand}, J.} \&
  {{Stadel}, J.}, astro-ph/0608495
  (2006),


%% AP_EDRFs %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% AP_EMFs %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{VoelkAtoyan2000}
{{V{\"o}lk}, H.~J.},\& {{Atoyan}, A.~M.}
newblock {\apj} {\bf 541}, 88 (2000),

%{END REFERENCES FOR ESWG02}

%BEGIN REFERENCES FOR GRB}

\bibitem{Hurleyetal94}K. Hurley et al., 1994, Nature 372, 652

\bibitem{Dingus95}B. L. Dingus, 1995, Astrophys.\ Space Sci.\ 231, 187

\bibitem{Dingusetal98}B. L. Dingus, J. R. Catelli, \& E. J. Schneid, 1998, AIP Conf.\ Proc.\ 428, 349 

\bibitem{Gonzalezetal03}M. M. Gonz\'alez et al., 2003, Nature 424, 749

\bibitem{Atkinsetal00}R. Atkins et al., 2000, Astrophys.\ J.\ Lett.\ 533, L119

\bibitem{Atkinsetal03}R. Atkins et al., 2003, Astrophys.\ J. 583, 824

\bibitem{Paczynski86}  Paczy\'nski, B. 1986, Astrophys.\ J., 308, L43

\bibitem{Goodman86}  Goodman, J. 1986, Astrophys.\ J., 308, L43

\bibitem{Paczynski90}   Paczy\'nski, B. 1990, Astrophys.\ J., 363, 218

\bibitem{PaczynskiXu94}  Paczy\'nski, B., \& Xu, G. 1994, Astrophys.\ J., 427, 708

\bibitem{ReesMeszaros94}  Rees, M.J., \& M\'esz\'aros, P. 1994, Astrophys.\ J., 430, L93

\bibitem{ReesMeszaros92}  Rees, M.J., \& M\'esz\'aros, P. 1992, Mon.\ Not.\ Roy.\ Astron.\ Soc., 258, 41

\bibitem{DermerMitman99}   Dermer, C.D., \& Mitman, K.E. 1999, Astrophys.\ J., 513, L5

%Reference revised and moved earlier in list
\bibitem{Dermer07}Dermer, C. 2007, Astrophys.\ J., 664, 384

\bibitem{Kazimuraetal98}  Kazimura, Y., et al.\  1998, Astrophys.\ J., 498, L183

\bibitem{Silvaetal03}  Silva, L.O., et al.\  2003, Astrophys.\ J., 596, L121

\bibitem{Frederiksenetal04}   Frederiksen, J.T., et al.\  2004, Astrophys.\ J., 608, L13

\bibitem{Nishikawaetal05}  Nishikawa, K.-I., et al.\  2005, Astrophys.\ J., 622, 927

%Reference added
\bibitem{Spitkovsky08} Spitkovsky, A.\  2008, arXiv:0802.3216

\bibitem{PanaitescuMeszaros98} Panaitescu, A., \& M\'esz\'aros, P. 1998, Astrophys.\ J., 492, 683

\bibitem{Thompson94}   Thompson, C. 1994, Mon.\ Not.\ Roy.\ Astron.\ Soc., 270, 480

\bibitem{Usov94}  Usov, V. V. 1992, Nature, 357, 472 

\bibitem{MeszarosRees97}   M\'esz\'aros, P., \& Rees, M.J. 1997, Astrophys.\ J., 482, L29

\bibitem{Drenkhahn02}   Drenkhahn, G. 2002, A\&A, 387, 714

\bibitem{DrenkhahnSpruit02}   Drenkhahn, G., \& Spruit, H. 2002, A\&A, 391, 1141

\bibitem{LyutikovBlandford03}   Lyutikov, M., \& Blandford, R. 2003, astro-ph/0312347

\bibitem{GianniosSpruit05}   Giannios, D., \& Spruit, H. 2005, A\&A, 430, 1   

\bibitem{Kumar99}   Kumar, P. 1999, Astrophys.\ J., 523, L113

\bibitem{Panaitescuetal99}   Panaitescu, A., Spada, M., \& M\'esz\'aros, P. 1999, Astrophys.\ J., 522, L105

\bibitem{Meszarosetal93}  M\'esz\'aros, P., Laguna, P., \& Rees, M.J. 1993, Astrophys.\ J., 415, 181

\bibitem{MeszarosRees93b}  M\'esz\'aros, P., \& Rees, M.J. 1993, Astrophys.\ J., 418, L59

\bibitem{Katz94b}   Katz, J.I. 1994, Astrophys.\ J., 432, L107

%\bibitem{MedvedevLoeb99}   Medvedev, M.V., \& Loeb, A. 1999, Astrophys.\ J., 526, 697

%\bibitem{PeerZhang06}  Pe'er, A., \& Zhang, B. 2006, Astrophys.\ J., 653, 454

%\bibitem{Hededaletal04}  Hededal, C.B., et al.\  2004, Astrophys.\ J., 617, L107

%\bibitem{Nishikawaetal06}   Nishikawa, K.-I., et al.\  2006, Astrophys.\ J., 642, 1267

\bibitem{PeerWaxman04b}  Pe'er, A., \& Waxman, E. 2004, Astrophys.\ J., 613, 448

\bibitem{Tavani96a}  Tavani, M. 1996, Astrophys.\ J., 466, 768

\bibitem{Tavani96b}  Tavani, M. 1996, Phys.\ Rev.\ Lett., 76, 3478

\bibitem{Cohenetal97}   Cohen, E., et al.\  1997, Astrophys.\ J., 488, 330

\bibitem{Crideretal97}  Crider, A., et al.\  1997, Astrophys.\ J., 479, L39

\bibitem{Preeceetal98}  Preece, R.D., et al.\  1998, Astrophys.\ J., 506, L23

\bibitem{Fronteraetal00}  Frontera, F., et al.\  2000, Astrophys.\ J.s, 127, 59

\bibitem{Preeceetal02}  Preece, R.D., et al.\  2002, Astrophys.\ J., 581, 1248

%Reference revised
\bibitem{Ghirlandaetal03}   Ghirlanda, G., Celotti, A., \& Ghisellini, G. 2003, A\&A, 406, 879 

\bibitem{Medvedev00}   Medvedev, M.V. 2000, Astrophys.\ J., 540, 704

\bibitem{LloydPetrosian00}  Lloyd, N.M., \& Petrosian, V. 2000, Astrophys.\ J. 543, 722

\bibitem{LloydRonningPetrosian02}   Lloyd-Ronning, N.M., \& Petrosian, V. 2002, Astrophys.\ J., 565, 182

\bibitem{DermerBoettcher00}   Dermer, C.D., \& B\"ottcher, M. 2000, Astrophys.\ J., 534, L155

\bibitem{Granotetal00} Granot, J., Piran, T., Sari 2000, Astrophys.\ J., 534, L163

\bibitem{MeszarosRees00}  M\'esz\'aros, P., \& Rees, M.J. 2000, Astrophys.\ J., 530, 292

\bibitem{DaigneMochkovitch02}  Daigne, F., \& Mochkovitch, R. 2002, Mon.\ Not.\ Roy.\ Astron.\ Soc., 336, 1271

\bibitem{Meszarosetal02}   M\'esz\'aros, P., Ramirez-Ruiz, E., Rees, M.J., \& Zhang, B. 2002, Astrophys.\ J., 578, 812

\bibitem{Ryde04}  Ryde, F. 2004, Astrophys.\ J., 614, 827

\bibitem{Ryde05}  Ryde, F. 2005, Astrophys.\ J.l, 625, L95

\bibitem{MeszarosRees94}  M\'esz\'aros, P., \& Rees, M.J. 1994, Mon.\ Not.\ Roy.\ Astron.\ Soc., 269, L41

\bibitem{Meszarosetal94}  M\'esz\'aros, P., Rees, M.J., \& Papathanassiou, H. 1994, Astrophys.\ J., 432, 181

\bibitem{PapathanassiouMeszaros96}  Papathanassiou, H., \& M\'esz\'aros, P. 1996, Astrophys.\ J., 471, L91

\bibitem{Liangetal97}   Liang, E. P., Kusunose, M., Smith, I., \& Crider, A. 1997, Astrophys.\ J., 479, L35 

\bibitem{SariPiran97}  Sari, R., \& Piran, T. 1997, Mon.\ Not.\ Roy.\ Astron.\ Soc., 287, 110

\bibitem{PillaLoeb98}  Pilla, R.P., \& Loeb, A. 1998, Astrophys.\ J., 494, L167

\bibitem{ChiangDermer99}  Chiang, J., \& Dermer, C.D. 1999, Astrophys.\ J., 512, 699

\bibitem{PanaitescuMeszaros00}   Panaitescu, A., \& M\'esz\'aros, P. 2000, Astrophys.\ J., 544, L17

%Reference added
\bibitem{BaringBraby04}  Baring, M. \% Braby, M. 2004, Astrophys.\ J., 613, 460

\bibitem{ReesMeszaros05}  Rees, M.J., \& M\'esz\'aros, P. 2005, Astrophys.\ J., 628, 847

\bibitem{Peeretal06}  Pe'er, A.,  M\'esz\'aros, P., \& Rees, M.J. 2006, Astrophys.\ J., 642, 995

\bibitem{ShavivDar95}   Shaviv, N.J., \& Dar, A. 1995, Astrophys.\ J., 447, 863

\bibitem{Lazzatietal00}  Lazzati, D., Ghisellini, G., Celotti, A., \& Rees, M.J. 2000, Astrophys.\ J.,
529, L17

\bibitem{Broderick05}  Broderick, A.E. 2005, Mon.\ Not.\ Roy.\ Astron.\ Soc., 361, 955

\bibitem{Inoueetal03}   Inoue, S., Guetta, D., \& Pacini, F. 2003, Astrophys.\ J., 583, 379

\bibitem{Liang97}   Liang, E. P. 1997, Astrophys.\ J., 491, L15  

\bibitem{GhiselliniCelotti99}   Ghisellini, G., \& Celotti, A. 1999, Astrophys.\ J., 511, L93

%\bibitem{Peeretal05}   Pe'er, A.,  M\'esz\'aros, P., \& Rees, M.J. 2005, Astrophys.\ J., 635, 476

\bibitem{GuettaGranot03a}   Guetta, D., \& Granot, J. 2003, Astrophys.\ J., 585, 885

\bibitem{GranotGuetta03a}  Granot, J., \& Guetta, D. 2003, Astrophys.\ J., 598, L11

\bibitem{PeerWaxman04a}   Pe'er, A., \& Waxman, E. 2004, Astrophys.\ J., 603, L1

%\bibitem{PeerWaxman05b}  Pe'er, A., \& Waxman, E. 2005, Astrophys.\ J., 633, 1018

\bibitem{KrolikPier91}  Krolik, J. H., \& Pier, E.A. 1991, Astrophys.\ J., 373, 277

\bibitem{FenimoreEpsteinHo93}  Fenimore, E.E., Epstein, R.I., \& Ho, C. 1993, A\&A, 97, 59 

\bibitem{WoodsLoeb95}   Woods, E., \& Loeb, A. 1995, Astrophys.\ J., 453, 583

\bibitem{BaringHarding97}   Baring, M.G., \& Harding, A.K. 1997, Astrophys.\ J., 491, 663

\bibitem{LithwickSari01}  Lithwick, Y., \& Sari, R. 2001, Astrophys.\ J., 555, 540

\bibitem{Razzaqueetal04}  Razzaque, S.,   M\'esz\'aros, P., \& Zhang, B. 2004, Astrophys.\ J., 613, 1072

\bibitem{KobayashiZhang03}   Kobayashi, S., \& Zhang, B. 2003, Astrophys.\ J., 597, 455

\bibitem{Zhangetal03}  Zhang, B., Kobayashi, S. \& M\'asz\'aros, P. 2003, Astrophys.\ J., 595, 950

%Reference revised
\bibitem{Peeretal07}   Pe'er, A. et al. 2007, Astrophys.\ J., 664, L1

%Reference added
\bibitem{GuptaZhang08} Gupta, N., Zhang, B., 2008, Mon.\ Not.\ Roy.\ Astron.\ Soc., 384, L11

%\bibitem{Svensson84}   Svensson, R. 1984, Mon.\ Not.\ Roy.\ Astron.\ Soc., 209, 175 

%\bibitem{PeerWaxman05a}   Pe'er, A., \& Waxman, E. 2005, Astrophys.\ J., 628, 875

\bibitem{Vietri97}   Vietri, M. 1997, Phys. Rev. Lett., 78, 4328

\bibitem{BottcherDermer98}  B\"ottcher, M., \& Dermer, C.D. 1998, Astrophys.\ J., 499, L131

\bibitem{Totani98}   Totani, T. 1998, Astrophys.\ J., 509, L81

\bibitem{WaxmanBahcall97}  Waxman, E., \& Bahcall, J. 1997, Phys. Rev. Lett., 78, 2292

\bibitem{WaxmanBahcall00}   Waxman, E., \& Bahcall, J. 2000, Astrophys.\ J., 541, 707

\bibitem{DermerAtoyan03}  Dermer, C.D., \& Atoyan, A.  2003, Phys.\ Rev.\ Lett., 91, 071102 

\bibitem{GuettaGranot03b}    Guetta, D., \& Granot, J. 2003, Phys. Rev. Lett., 90, 1103

\bibitem{GranotGuetta03b}   Granot, J., \& Guetta, D. 2003, Phys. Rev. Lett., 90, 1119

%Reference revised
\bibitem{Dermeretal07}   Dermer, C.D., Ramirez-Ruiz, E. \& Le, T. 2007, Astrophys.\ J., 664, L67

%\bibitem{Kazanasetal02}   Kazanas, D., Georganopoulos, M., \& Mastichiadis, A. 2002, Astrophys.\ J., 578, L15

%\bibitem{MastichiadisKazanas06}   Mastichiadis, A. \& Kazanas, D. 2006, Astrophys.\ J., 645, 416

\bibitem{Katz94a}  Katz, J.I. 1994, Astrophys.\ J., 432, L27

\bibitem{DePaolisetal00}   De Paolis, F., Ingrosso, G., \& Orlando, D. 2000, A\&A, 359, 514

\bibitem{Derishevetal99}  Derishev, E.V., Kocharovsky, V.V., \& Kocharovsky, Vl, V. 2001, Astrophys.\ J.,
521, 640

\bibitem{BahcallMeszaros00}   Bahcall, J.N., \& M\'esz\'aros, P. 2000, Phys.\ Rev.\ Lett., 85, 1362

\bibitem{Rossietal06}   Rossi, E., Beloborodov, A.M., \& Rees, M.J. 2006, Mon.\ Not.\ Roy.\ Astron.\ Soc., 369, 1797

%\bibitem{BlandfordMcKee76}   Blandford, R.D., \& McKee, C.F. 1976, Phys. Fluids, 19, 1130

%\bibitem{MeszarosRees93a}  M\'esz\'aros, P., \& Rees, M.J. 1993, Astrophys.\ J., 405, 278

%\bibitem{Sarietal98}   Sari, R., Piran, T., \& Narayan, R. 1998, Astrophys.\ J., 497, L17

%\bibitem{Wijersetal97}  Wijers, R.A.M.J., Rees, M.J., \& M\'esz\'aros, P.  1997, Mon.\ Not.\ Roy.\ Astron.\ Soc., 288, L51

%\bibitem{FreedmanWaxman01}  Freedman, D.L., \& Waxman, E. 2001, Astrophys.\ J., 547, 922

%\bibitem{Bergeretal03}   Berger, E., Kulkarni, S.R., \& Frail, D. 2003, Astrophys.\ J., 590, 379

%\bibitem{SariEsin01}   Sari, R., \& Esin, A.A. 2001, Astrophys.\ J., 548, 787

\bibitem{ReesMeszaros98}  Rees, M.J., \& M\'esz\'aros, P. 1998, Astrophys.\ J., 496, L1

\bibitem{Granotetal03}   Granot, J., Nakar, E., \& Piran, T. 2003, Nature, 426, 138

\bibitem{KumarPiran00}   Kumar, P., \& Piran, T. 2000, Astrophys.\ J., 535, 152 

\bibitem{WangLoeb00}  Wang, X., \& Loeb, A. 2000, Astrophys.\ J., 535, 788 

\bibitem{Nakaretal03}   Nakar, E., Piran, T., \& Granot, J. 2003, NewA, 8, 495

\bibitem{Wijers01}  Wijers, R.A.M.J. 2001, in Gamma Ray Bursts in the Afterglow Era,
ed. E. Costa, Frontera. F. and Hjorth J. (Springer: Berlin) 306 

\bibitem{RamirezRuizetal05}  Ramirez-Ruiz, E., Garc\'ia-Segura, G., Salmonson, J.D., \&
P\'erez-Rend\'on, B. 2005, Astrophys.\ J., 631, 435

\bibitem{PeerWijers06}   Pe'er, A., \& Wijers, R.A.M.J. 2006, Astrophys.\ J., 643, 1036

\bibitem{NakarGranot07} Nakar, E. \& Granot, J. 2007, Mon.\ Not.\ Roy.\ Astron.\ Soc., 380, 1744

%Reference revised
\bibitem{Genetetal07}  Genet, F., Daigne, F., \& Mochkovitch, R. 2007, Mon.\ Not.\ Roy.\ Astron.\ Soc., 381, 732

%Reference revised
\bibitem{UhmBeloborodov07}   Uhm, Z., \& Beloborodov, A. 2007, Astrophys.\ J., 665, 93

%\bibitem{FryerWoosley98} C. L. Fryer  \& S. E. Woosley, 1998, Astrophys.\ J. 502, L9

%\bibitem{Fryeretal07} C. L. Fryer,  et al., 2007, submitted to Astrophys.\ J., astro-ph/0702338

%\bibitem{PanaitescuMeszaros06} A. Panaitescu, P. Meszaros, N. Gehrels, D. Burrows \& J. Nousek,  2006, Mon.\ Not.\ Roy.\ Astron.\ Soc.\ 366, 1357

%\bibitem{FryerYoung06}C. L. Fryer, P. A. Young, A. L. Hungerford, 2006, Astrophys.\ J. 650, 1028

%%DAW0301 DAW Start of references for GRB observations section

%\bibitem{Aharonian:07:ICRCGRBs} Aharonian, F., et al. 2007, Paper 464,
%Proc. 30th ICRC, Merida, Mexico

\bibitem{Padilla:98:Airobicc} Padilla, L., et al. 1998, A\&A, 337, 43

\bibitem{Amenomori:01:TibetGRBs} Amenomori, M., et al. 2001, AIP
Conf. Proc., 558, 844

\bibitem{Atkins:05:MilagroGRBCounterparts} Atkins, R., et al. 2005,
ApJ, 630, 996

%Reference revised
\bibitem{SazParkinson:07:MilagroGRBCounterparts} Saz Parkinson, P. M. 2007, AIP Conf.\ Proc.\ 921, 470

\bibitem{Abdo:07:MilagroGRBCounterparts} Abdo, A. A., et al. 2007,
ApJ, 666, 361

\bibitem{Atkins:04:MilagroGRB} Atkins, R., et al. 2004, ApJ, 604, L25

\bibitem{Meegan:92} Meegan, C. A., et al. 1992, Nature, 355, 143

\bibitem{Connaughton:97} Connaughton, V., et al. 1997, ApJ, 479, 859

\bibitem{Horan:07} Horan, D., et al. 2007, ApJ, 655, 396

\bibitem{Albert:06:40sGRB} Albert, J., et al. 2006, ApJ, 641, L9

\bibitem{Bastieri:07:ICRCStatus} Bastierei, D., et al. 2007,
Proc. 30th ICRC Merida, Mexico, ArXiv e-prints 0709.1380

%Reference revised
\bibitem{Albert:2006:GRBs} Albert, J., et al. 2007,  Astrophys.\ J. 667, 358

\bibitem{Bastieri:7:ICRCGRBObs} Bastierei, D., et al. 2007b,
Proc. 30th ICRC Merida, Mexico, ArXiv e-prints 0709.1386

\bibitem{Horan:07ICRC} Horan, D., et al. 2007b, Paper 406, Proc. 30th
ICRC, Merida, MX

%\bibitem{Aharonian06:PG1553} Aharonian, F., et al. 2006, A\&A, 448,
%L19

%\bibitem{Treves:07} Treves, A., Falomo, R. \& Uslenghi, M. 2007, A\&A
%Letters (in press), ArXiv e-prints 0709.1271

%Reference revised
\bibitem{Teshima:07} Albert, J., et al. 2008, Science, 27, 1752

%%DAW not used? \bibitem{Connaughton:02} Connaughton, V. 2002, ApJ, 567, 1028

%%DAW End of references for GRB observations section

\bibitem{Woosley93} Woosley, S. E. 1993, Astrophys.\ J., 405, 273

\bibitem{MacFadyenWoosley99} MacFadyen, A. I. \& Woosley, S. E. 1999, Astrophys.\ J., 524, 262

\bibitem{Bloometal99} Bloom, J. S. et al. 1999, Nature, 401, 453

\bibitem{Haislipetal06} Haislip, J. B. et al. 2006, Nature, 440, 181

\bibitem{Bergeretal05a} Berger, E. et al. 2005, Astrophys.\ J., 634, 501

\bibitem{Jakobssen06} Jakobssen, P.,  Levan, A., Fynbo, J.P.U., et al. 2006, Astron. \& Astrophys., 447, 897

\bibitem{Campanaetal06} Campana, S. et al. 2006, Nature, 442, 1008

%Reference revised
\bibitem{GuptaZhang07} Gupta, N., Zhang, B., 2007, Mon.\ Not.\ Roy.\ Astron.\ Soc., 380, 78

%Reference added
\bibitem{Racusin08} Racusin, J. L. et al. 2008, Nature, 455, 183

%\bibitem{Baring06} Baring, M. G. 2006, Astrophys.\ J., 650, 1004

%Reference revised
\bibitem{Granotetal08} Granot, J., Cohen-Tanugi, J., do Couto e Silva, E. 2008, Astrophys.\ J., 677, 92

%\bibitem{PanaitescuKumar02} Panaitescu, A. \& Kumar, P. 2002, Astrophys.\ J., 571, 779

%\bibitem{Mundelletal07} Mundell et al. 2006, Astrophys.\ J., in press (astro-ph/0610660)

%\bibitem{Schadyetal07} Schady, P. et al. 2006a, Mon.\ Not.\ Roy.\ Astron.\ Soc., submitted (astro-ph/0611081)

%Reference revised
\bibitem{Molinarietal07} Molinari, E. et al. 2007, A\&A, 469, 13

\bibitem{DardeRujula04} Dar, A., \& de
R{\'u}jula, A.\ 2004, Phys.\ Rep., 405, 203

\bibitem{DadoDar05} Dado, S., \& Dar, A.\
2005, Astrophys.\ J.\ Lett., 627, L109

%\bibitem{Casanovaetal07} Casanova, S., Dingus, B., Zhang, B., 2007, Astrophys.\ J., 656, 306

\bibitem{ZhangMeszaros01} Zhang, B., M\'esz\'aros P. 2001, Astrophys.\ J., 559, 110

\bibitem{Dermeretal00}   Dermer, C.D., Chiang, J., \& Mitman, K.E. 2000, Astrophys.\ J., 537, 785

\bibitem{Wangetal01a} Wang, X. Y., Dai, Z. G., Lu, T. 2001, Astrophys.\ J., 546, L33

\bibitem{Wangetal01b} Wang, X. Y., Dai, Z. G., Lu, T. 2001, Astrophys.\ J., 556, 1010

\bibitem{Romingetal06} Roming, P. et al. 2006, Astrophys.\ J., 652, 1416

\bibitem{Zhangetal06} Zhang, B. et al., 2006, Astrophys.\ J., 642, 354

\bibitem{Nouseketal06} Nousek, J. A. et al. 2006, Astrophys.\ J., 642, 389

\bibitem{Tagliaferrietal05} Tagliaferri, G. et al. 2005, Nature, 436, 985

\bibitem{KumarPanaitescu00} Kumar, P. \& Panaitescu, A. 2000, Astrophys.\ J., 541, L51

\bibitem{Meszaros06} M\'esz\'aros, P. 2006, Rev.\ Prog.\ Phys., 2006, 69, 2259

%Reference revised
\bibitem{Granot06} Granot, J. 2006, Il Nuovo Cimento B, 121, 1073

\bibitem{Zhang07} Zhang, B. 2007, ChJAA, 7, 1

\bibitem{Panaitescuetal06a} Panaitescu, A. et al. 2006, Mon.\ Not.\ Roy.\ Astron.\ Soc., 366, 1357

\bibitem{GranotKumar06} Granot, J. \& Kumar, P. 2006, Mon.\ Not.\ Roy.\ Astron.\ Soc., 366, L13

\bibitem{KobayashiZhang07} Kobayashi, S. \& Zhang, B. 2007, Astrophys.\ J., 655, 973

\bibitem{EichlerGranot06} Eichler, D. \& Granot, 2006, Astrophys.\ J., 641, L5

\bibitem{Granotetal06} Granot, J., K\"onigl, A. \& Piran, T. 2006, Mon.\ Not.\ Roy.\ Astron.\ Soc., 370, 1946

\bibitem{Iokaetal06} Ioka, K., Toma, K., Yamazaki, R. \& Nakamura, T. 2006, A\&A, 458, 7

\bibitem{Panaitescuetal06b} Panaitescu, A. et al. 2006, Mon.\ Not.\ Roy.\ Astron.\ Soc., 369, 2059

%Reference revised
\bibitem{GouMeszaros07} Gou, L. J. \& M\'esz\'aros, P. 2007, Astrophys.\ J., 668, 392

%Reference revised
\bibitem{Fanetal07} Fan, Y. et al. 2007, Mon.\ Not.\ Roy.\ Astron.\ Soc., 384, 1483

\bibitem{Burrowsetal05} Burrows, D. N. et al. 2005, Science, 309, 1833

%Reference revised
\bibitem{Chincarinietal07} Chincarini, G. et al. 2007, Astrophys.\ J., 671, 1903

%Reference revised
\bibitem{Falconeetal07} Falcone, A. D. et al., 2007, Astrophys.\ J., 671, 1921

\bibitem{Falconeetal06} Falcone, A. D. et al., 2006, Astrophys.\ J., 641, 1010

\bibitem{Liangetal06} Liang, E. W. et al. 2006, Astrophys.\ J., 646, 351

\bibitem{Wangetal06} Wang, X.-Y., Li, Z., M\'esz\'aros, P. 2006, Astrophys.\ J., 641, L89

%\bibitem{RazzaqueMeszaros06b} Razzaque, S., \& M\'esz\'aros, P. 2006, JCAP, 06, 006

\bibitem{Primacketal99} Primack, J. R. et al. 1999, APh, 11, 93

\bibitem{Steckeretal06} Stecker, F. W., Malkan M. A.  \& Scully S. T.  2006., Astrophys.\ J., 648, 774

\bibitem{ChengCheng96} Cheng, L. X., \& Cheng, K. S. 1996, Astrophys.\ J., 459, L79

\bibitem{DaiLu02} Dai, Z. G., Lu, T. 2002, Astrophys.\ J., 580, 1013

\bibitem{Wangetal04} Wang, X. Y., Cheng, K. S., Dai, Z. G., Lu, T. 2004, Astrophys.\ J., 604, 306

\bibitem{Plaga95} Plaga, R. 1995, Nature, 374, 430

\bibitem{Gehrelsetal05} Gehrels, N. et al. 2005, Nature, 437, 851

\bibitem{Foxetal05} Fox, D. B. et al. 2005, Nature, 437, 845

\bibitem{Barthelmyetal05} Barthelmy, S. D. et al. 2005, Nature, 438, 994

\bibitem{Bergeretal05b} Berger, E. et al. 2005, Nature, 438, 988

%Reference added
\bibitem{Bloometal06} Bloom, J. S. et al. 2006, Astrophys.\ J., 638, 354

\bibitem{Gehrelsetal06} Gehrels, N. et al. 2006, Nature, 444, 1044

\bibitem{Zhangetal07} Zhang, B. et al. 2007, Astrophys.\ J., 655, L25

\bibitem{WangMeszaros06}Wang, X. Y., \& M\'esz\'aros, P. 2006, Astrophys.\ J., 643, L95

%Reference revised
\bibitem{Waxmanetal07} Waxman, E.,  M\'esz\'aros, P. \& Campana, S., 2007, Astrophys.\ J., 667, 351

%\bibitem{Totani98b} Totani, T. 1998, Astrophys.\ J., 502, L13

\bibitem{Waxman95} E. Waxman 1995, Phys.\ Rev.\ Lett., 75, 386

\bibitem{Vietri95} M. Vietri 1995, Astrophys.\ J., 453, 883

\bibitem{Dermer02} C. D. Dermer 2002, Astrophys.\ J., 574, 65

%\bibitem{ShemiPiran90} A. Shemi and T. Piran 1990, Astrophys.\ J., 365, L55

%\bibitem{MeszarosRees97b} P. M\'esz\'aros and M. J. Rees 1997, Astrophys.\ J., 476, 232

%\bibitem{Dermeretal99} C. D. Dermer, M. B\"ottcher and J. Chiang 1999, Astrophys.\ J.,  515, L49

\bibitem{Vietri98} M. Vietri 1998, Astrophys.\ J., 507, 40

\bibitem{DermerHumi01} C. D. Dermer and M.\ Humi 2001, Astrophys.\ J.,   479, 493

\bibitem{RazzaqueMeszaros06a} Razzaque, S., \& M\'esz\'aros, P. 2006, Astrophys.\ J., 650, 998

\bibitem{Abdoetal07} Abdo, A. A. et al. 2007, Astrophys.\ J., 666, 361

%\bibitem{Beloborodov03} A. M. Beloborodov 2003, Astrophys.\ J.,  588, 931

\bibitem{RachenMeszaros98} J. P. Rachen and P. M\'esz\'aros 1998, Phys.\ Rev.\ D,  58, 123005

\bibitem{AtoyanDermer03} A. Atoyan and C. D. Dermer 2003, Astrophys.\ J.,   586, 79

\bibitem{DermerAtoyan04} C. D. Dermer and A. Atoyan 2004, Astron.\ Ap., 418, L5

\bibitem{Totani99} T. Totani 1999, Astrophys.\ J.,  511, 41

\bibitem{Fragileetal04} Fragile, P. C., Mathews, G. J., Poirier, J. \& Totani, T. 2004, APh, 20, 591

\bibitem{Wangetal05} X. Y. Wang, K. S. Cheng, Z. G. Dai and T. Lu 2005, Astron.\ Ap.,  439, 957

\bibitem{WaxmanCoppi96} E. Waxman and P. Coppi 1996, Astrophys.\ J., 464, L75

%\bibitem{Razzaqueetal04b} S. Razzaque, P. M\'esz\'aros and E. Waxman 2004, Phys.\ Rev.\ D,  69, 023001

%\bibitem{Guettaetal04} D. Guetta, D. Hooper, J. Alvarez-Muniz, F. Halzen and E. Reuveni 2004, Astropart.\ Phys.,  20, 429

%\bibitem{Ellisetal03} Ellis, J., et al.  2003, Astron.\ Ap., 402, 409

%\bibitem{Fenimoreetal95} Fenimore, E.E., et al. 1995, Astrophys.\ J., 448, 101

%\bibitem{Norrisetal96} Norris, J.P., et al.  1996, Astrophys.\ J., 459, 393

%\bibitem{Norrisetal05} Norris, J.P., et al.  2005, Astrophys.\ J., 627, 324

%\bibitem{NorrisBonnell06} Norris, J.P., \& Bonnell, J.T.  2006, Astrophys.\ J., 643, 266

\bibitem{ellis1992} Ellis, J.R., Mavromatos, N.E., \& Nanopoulos, D.V. 1992, Phys. Lett. B, 293, 37

\bibitem{amelino1997} Amelino-Camelia, G., Ellis, J.R., Mavromatos, N.E., \& Nanopoulos, D.V. 1997, Int. J. Mod. Phys. A, 12, 607

\bibitem{gambini1999} Gambini, R. and Pullin, J. 1999, Phys. Rev. D, 59

%Reference revised
\bibitem{albert2007} Albert, J. et al. [MAGIC collaboration] 2008, Phys. Lett. B, in press 

%Reference revised
\bibitem{Scargleetal07} Scargle, J., Norris, J., \& Bonnell, J. 2007, Astrophys.\ J., 673, 972

%Reference removed
%\bibitem{albertetal08} Albert, J. et al. [MAGIC collaboration] 30th International Cosmic Ray Conference, Merida, July 2007; arXiv:0709.1475

\bibitem{PeerWaxman05b}  Pe'er, A., \& Waxman, E. 2005, Astrophys.\ J., 633, 1018

%Reference revised
\bibitem{Franceschinietal2008} Franceschini, A., Rodighiero, G., Vaccari, M. 2008, Astron. \& Astrophys., 487, 837

%Reference revised
\bibitem{KowalskiMohr07}Kowalski, M. \& Mohr, A. 2007, Astropart.\ Phys., 27, 533

%Reference revised
\bibitem{Achterbergetal07} Achterberg, A. et al. 2008, Astrophys.\ J., 674, 357

%Reference added
\bibitem{StamatikosBand06} Stamatikos, M. \& Band, D. L. 2006, AIP Conf.\ Proc.\ 836, 599

%{END REFERENCES FOR GRB}

%{Begin REFERENCES FOR WPTECH}

\bibitem{1989ApJ...342..379W} T.\ C. \ Weekes  et al., \apj, 342,  379  (1989).

\bibitem{Week:02}{Weekes, T.\ C., Badran, H., Biller, S.\ D., et al., APh, 17, 221\ (2002)}

\bibitem{Maie:07} {Maier, G. et al.\ 2007, In Proc.\ 30th International Cosmic Ray Conference, Merida, Mexico, (2007)}

\bibitem{2004NewAR..48..339L} E. Lorenz, NewAR, {\bf 48},  339  (2004).
\bibitem{Goeb:07}{Goebel, F. et al., arXiv:0709.2032 (2007)}
\bibitem{2004NewAR..48..331H}J.~A. Hinton, NewAR, {\bf 48},  331  (2004).

\bibitem{Horn:07}{Horns, D. et al.\, Journal of Physics Conference 
Series, 60, 119 (2007)}
\bibitem{Smit:05}{Smith, A.J. et al., Proceedings of 29th ICRC, 10, 227 (2005)} 
\bibitem{Abdo:07}{Abdo, A. A., Allen, B., Berley, D., ApJL, 664, 91 (2007)}
	
\bibitem{2007ebhe.conf..282W}{Weekes, T.\ C., Proc. of Energy Budget in the High Energy Universe
workshop, Eds.\ K.\ Sato \& J.\ Hisano, p.282 (2007)}

\bibitem{Mori:07}{Mori, M. et al.\ 2007, In Proc.\ 30th International Cosmic Ray Conference, Merida, Mexico, (2007)}

\bibitem{Zao:05}{Aielli G., el al., Nuclear Physics B . Proceedings 
Supplements, 166, 96 (2007)} 

\bibitem{McEn:07}{McEnery, J. et al.\, In Proceedings of the 30th ICRC, 
Merida, Mexico (2007)}
\bibitem{Lich:07}{Lichti, G. G., et al.\, American Institute of Physics 
Conference Series, 906, 119 (2007)}
\bibitem{AharT:05}{Aharonian, F.\, In Proc.\ ``Towards a Network of 
Atmospheric Cherenkov Detectors VII'', Palaiseau, France,  arXiv:astro-ph/0511139 (2005)}
\bibitem{AharT:08}{Aharonian, F., Buckley, J., Sinnis, G.\, RoP, in 
press. (2008)}
\bibitem{Hofmann2005} Hofmann, W., ``Performance Limits for 
Cherenkov Instruments., 2005, Palaiseau, France, arXiv:astro-ph/0603076v2, (2005)
\bibitem{VF2005} Vassiliev V.,\ V.\ \& Fegan, S.\ J., Palaiseau, France, 
arXiv:astro-ph/0511342v1, (2005)
\bibitem{FV2007} Fegan, S.\ J.,\ \& Vassiliev, V.\ V.,  In Proc.\ 30th 
ICRC, Merida, Mexico (2007)
\bibitem{Bugaev:07}{Bugaev, V. V., Buckley, J. H., Krawczynski, H.,
In Proceedings of the 30th ICRC, Merida, Mexico} (2007)
\bibitem{Krawcz:06}{Krawczynski, H., Carter-Lewis, D. A., Duke, C., et 
al., APh, 25, 380} (2006)
\bibitem{GLAST} {http://www-glast.slac.stanford.edu,
local link software/IS/glast\_lat\_performance.htm} 
\bibitem{FK:1995}{Krennrich, F., and Lamb, R.C., Experimental Astronomy, 
6, 285} (1995)
\bibitem{JKBF2005} Jung, I., et al., in ``Towards a Network of 
Atmospheric Cherenkov Detectors VII'',  Eds.\ B.\ Degrange \&  G.\ Fontaine, 
463 (2005)
\bibitem{stamatescu07} Stamatescu, V., In Proc. \ 30th ICRC, Merida, Mexico (2007); 
in ``towards a Network of Atmospheric Cherenkov 
Detectors VI
I'',  Eds.\ B.\ Degrange and G.\ Fontaine, 445 (2007)
\bibitem{SC:1905} {\ Schwarzschild, K., Astronomische Mittheilungen der 
K\"oniglichen Sternwarte zu G\"ottingen, 10, 3} (1905)
\bibitem{Vass:07}{Vassiliev, V., Fegan, S., Brousseau, P., APh, 28, 
10} (2007)
\bibitem{Schwarzschild1905}{Schwarzschild}, K., Untersuchungen zur 
geometrischen Optik II (1905)
\bibitem{Smith_GLAST:07}{Smith, A.J. et al., {\em Proceedings of the 
1st GLAST Science Symposium}, AIP Vol 921, eds. S. Ritz, P. Michelson, C. Meegan, 
442} (2007)
\bibitem{dingus:07} {Dingus, B. L. et al., {\em Proceedings of the 1st 
GLAST  Science Symposium}, AIP Vol 921, eds. S. Ritz, P. Michelson, C. Meegan, 
438} (2007)
\bibitem{Sinnis2004} Sinnis, G., Smith, A., and McEnery, J. E., {\em 
Proceedings of the 10th Marcel Grossman Meeting}, eds. M. Novello, S.P.Bergliaffa,  \& 
R. Ruffini, 1068 (2004)
\bibitem{Sinnis2005} Sinnis, G., {\em proceedings Towards A Network of 
Atmospheric Cherenkov Telescopes VII}, Palaiseau, France (2005)

%{END REFERENCES FOR WPTECH}

\end{thebibliography}

